A Simple Adaptive Procedure Converging to Forgiving Correlated Equilibria

Simple adaptive procedures that converge to correlated equilibria are known to exist for normal form games (Hart and Mas-Colell 2000), but no such analogue exists for extensive-form games. Leveraging inspiration from Zinkevich et al. (2008), we show that any internal regret minimization procedure designed for normal-form games can be efficiently extended to finite extensive-form games of perfect recall. Our procedure converges to the set of forgiving correlated equilibria, a refinement of various other proposed extensions of the correlated equilibrium solution concept to extensive-form games (Forges 1986a; Forges 1986b; von Stengel and Forges 2008). In a forgiving correlated equilibrium, players receive move recommendations only upon reaching the relevant information set instead of all at once at the beginning of the game. Assuming all other players follow their recommendations, each player is incentivized to follow her recommendations regardless of whether she has done so at previous infosets. The resulting procedure is completely decentralized: players need neither knowledge of their opponents' actions nor even a complete understanding of the game itself beyond their own payoffs and strategies.

==> titlepage.tex <==
\begin{titlepage}
   \begin{center}
       \vspace*{1cm}

    \LARGE
       A Simple Adaptive Procedure\\
       Converging to Forgiving Correlated Equilibria \\
       \vspace{0.8cm}
        \large
       Hugh Zhang \\
       \vspace{0.05cm}
       Department of Economics \\
       \vspace{0.05cm}
       Stanford University \\
       
        \vspace{0.5cm}
       Undergraduate Honors Thesis \\
       \vspace{0.05cm}
       Advised by Gabriel Carroll \\
        \vspace{0.9cm}
    \textbf{Abstract}
    


    
   \end{center}
  \doublespacing

\noindent Simple adaptive procedures that converge to correlated equilibria are known to exist for normal form games \parencite{hart2000simple}, but no such analogue exists for extensive-form games.
Leveraging inspiration from \citeauthor{zinkevich2008regret} (\citedate{zinkevich2008regret}), we show that any internal regret minimization procedure designed for normal-form games can be efficiently extended to finite extensive-form games of perfect recall.
Our procedure converges to the set of forgiving correlated equilibria, a refinement of various other proposed extensions of the correlated equilibrium solution concept to extensive-form games \parencite{forges1986approach, forges1986correlated, von2008extensive}. 
In a forgiving correlated equilibrium, players receive move recommendations only upon reaching the relevant information set instead of all at once at the beginning of the game.
Assuming all other players follow their recommendations, each player is incentivized to follow her recommendations \emph{regardless of whether she has done so at previous infosets}.
The resulting procedure is completely decentralized: players need neither knowledge of their opponents' actions nor even a complete understanding of the game itself beyond their own payoffs and strategies.
%From a computational perspective, the procedures has polynomial runtime in the size of the game tree and converges at a rate of $O(\frac{1}{\sqrt{T}})$.
%Finally, we discuss variations of our procedure that use reduced memory or provide additional sequential rationality guarantees.
\\\\
\small
\textbf{Acknowledgements:} I am tremendously grateful to my advisor Gabriel Carroll for his support and guidance throughout the process of writing this thesis, as well as Marcelo Clerici-Arias for making this possible by directing the Economics Honors program. I would also like to thank Daniel Duckworth, Jeffrey Chang, Felix Wang, and Xiaoyu He for their helpful suggestions and comments, and my ECON 180 classmates for helping me learn game theory.

\end{titlepage}



